A Quarter of US-Trained Scientists Eventually Leave. Is the US Giving Away Its Edge?

Using newly-assembled data from 1980 through 2024, we show that 25% of scientifically-active, US-trained STEM PhD graduates leave the US within 15 years of graduating. Leave rates are lower in the life sciences and higher in AI and quantum science but overall have been stable for decades. Contrary to common perceptions, US technology benefits from these graduates' work even if they leave: though the US share of global patent citations to graduates' science drops from 70% to 50% after migrating, it remains five times larger than the destination country share, and as large as all other countries combined. These results highlight the value that the US derives from training foreign scientists - not only when they stay, but even when they leave.

==> tables/other/robust_gpt_maintech_2000_2019.tex <==
\begin{tabular}{lcc}
\hline
\hline
 Technology                                              &   Main Match (Full) &   Main Match (2\%) \\
\hline
 Biotechnologies                                         &                1756 &              1762 \\
 Advanced Engineering Materials                          &                1006 &               996 \\
 Semiconductors and Microelectronics                     &                 516 &               515 \\
 Advanced and Networked Sensing and Signature Management &                 369 &               369 \\
 Advanced Computing                                      &                 326 &               319 \\
 Clean Energy Generation and Storage                     &                 306 &               310 \\
 Artificial Intelligence                                 &                 300 &               295 \\
 Integrated Communication and Networking Technologies    &                 205 &               206 \\
 Advanced Manufacturing                                  &                 130 &               129 \\
 Quantum Information and Enabling Technologies           &                 108 &               108 \\
 Space Technologies and Systems                          &                  94 &                92 \\
 Highly Automated, Autonomous, and Uncrewed Systems      &                  64 &                64 \\
 Human-Machine Interfaces                                &                  42 &                39 \\
 Data Privacy, Data Security, and Cybersecurity          &                  32 &                30 \\
 Positioning, Navigation, and Timing (PNT) Technologies  &                  24 &                24 \\
 Directed Energy                                         &                  18 &                18 \\
 Advanced Gas Turbine Engine Technologies                &                  17 &                17 \\
 Hypersonics                                             &                   5 &                 5 \\
\hline
\hline
\end{tabular}


==> tables/other/robust_gpt_subtech_2000_2019.tex <==
\begin{tabular}{llcc}
\hline
\hline
 Technology                                    & Subfield                                                                       &   Match (Full) &   Match (2\%) \\
\hline
 Biotechnologies                               & Engineering of sub-cellular, multicellular, and multi-scale systems            &            775 &          785 \\
 Biotechnologies                               & Biotic/abiotic interfaces	                                                    &            728 &          717 \\
 Biotechnologies                               & Multi-omics, bioinformatics, and computational tools for phenotype analysis    &            345 &          343 \\
 Biotechnologies                               & Novel synthetic biology of nucleic acids, genome, epigenome, and protein design&            290 &          293 \\
 Biotechnologies                               & Engineering of viral and viral delivery systems                                &            127 &          128 \\
 Biotechnologies                               & Biomanufacturing and bioprocessing technologies                                &             85 &           88 \\
 Biotechnologies                               & Cell-free systems and technologies	                                            &             14 &           13 \\
 Artificial Intelligence                       & Machine learning                                                               &            273 &          267 \\
 Artificial Intelligence                       & Sensory perception and recognition                                             &             76 &           75 \\
 Artificial Intelligence                       & Deep learning                                                                  &             58 &           60 \\
 Artificial Intelligence                       & Reinforcement learning                                                         &             28 &           27 \\
 Artificial Intelligence                       & Technologies for improving AI safety, trust, security, and responsible use	    &             13 &           13 \\
 Artificial Intelligence                       & AI assurance and assessment techniques                                         &              5 &            4 \\
 Artificial Intelligence                       & Synthetic data approaches for training, tuning, and testing                    &              4 &            4 \\
 Artificial Intelligence                       & Foundation models                                                              &              2 &            3 \\
 Artificial Intelligence                       & Generative AI systems, multimodal and large language models                    &              2 &            2 \\
 Semiconductors and Microelectronics           & Beyond complementary metal-oxide-semiconductor (CMOS) technology               &            361 &          365 \\
 Semiconductors and Microelectronics           & Novel materials for advanced microelectronics                                  &            253 &          257 \\
 Semiconductors and Microelectronics           & Manufacturing process technologies and manufacturing equipment                 &            162 &          162 \\
 Semiconductors and Microelectronics           & Specialized hardware for AI, radiation, RF/optical, and high-power applications&            124 &          131 \\
 Semiconductors and Microelectronics           & Design and electronic design automation tools                                  &             62 &           63 \\
 Semiconductors and Microelectronics           & Microelectromechanical systems (MEMS) and Nanoelectromechanical systems (NEMS) &             61 &           60 \\
 Semiconductors and Microelectronics           & Heterogeneous integration and advanced packaging                               &             32 &           36 \\
 Semiconductors and Microelectronics           & Novel architectures for non-Von Neumann computing                              &             18 &           16 \\
 Quantum Information and Enabling Technologies & Materials, isotopes, and fabrication techniques for quantum devices            &             70 &           69 \\
 Quantum Information and Enabling Technologies & Quantum computing                                                              &             36 &           36 \\
 Quantum Information and Enabling Technologies & Quantum sensing                                                                &             25 &           26 \\
 Quantum Information and Enabling Technologies & Quantum communications and networking                                          &             11 &           13 \\
\hline
\hline
\end{tabular}

